Learning-Based Heavy Hitters and Flow Frequency Estimation in Streams

Identifying heavy hitters and estimating the frequencies of flows are fundamental tasks in various network domains. Existing approaches to this challenge can broadly be categorized into two groups, hashing-based and competing-counter-based. The Count-Min sketch is a standard example of a hashing-based algorithm, and the Space Saving algorithm is an example of a competing-counter algorithm. Recent works have explored the use of machine learning to enhance algorithms for frequency estimation problems, under the algorithms with prediction framework. However, these works have focused solely on the hashing-based approach, which may not be best for identifying heavy hitters. In this paper, we present the first learned competing-counter-based algorithm, called LSS, for identifying heavy hitters, top k, and flow frequency estimation that utilizes the well-known Space Saving algorithm. We provide theoretical insights into how and to what extent our approach can improve upon Space Saving, backed by experimental results on both synthetic and real-world datasets. Our evaluation demonstrates that LSS can enhance the accuracy and efficiency of Space Saving in identifying heavy hitters, top k, and estimating flow frequencies.

==> sections/removed.tex <==
We consider learning approaches to enhance Space Saving accuracy, called \lss{}.
Related work on predictions for algorithm design~\cite{gupta2016pac, dick2017data, balcan2018dispersion, hsu2019learning} introduced the concept of a heavy hitter predictor within the data stream which predicts whether it will be a heavy hitter or not.
It was shown that such a predictor can reduce the estimation errors of classical hash-based heavy hitter algorithms, such as Count-Min Sketch~\cite{cormode2005improved} and Count Sketch~\cite{charikar2002finding}.
Considering the advantages of the heavy hitter predictor when it comes to \emph{sketch-based} techniques~\cite{metwally2005efficient}, where multiple items can be mapped to the same bucket, an alternative approach is considered for \emph{counter-based} techniques.
Our approach incorporates two predictors: one for identifying low-frequency items and another for heavy hitters. To accommodate the availability of predictors in different systems, we divide \lss{} into two components: \lsslf{} when the low-frequency predictor is available and \lssasn{} when the heavy hitters predictor is available. When both predictors are available we use \lss{}.
\lsslf{} filters low-frequency items (single-occurrence items as a special case), resulting in a ``cleaner'' structure. Meanwhile, \lssasn{} uses heavy hitters predictor to allocate fixed entries for these items. Other items are processed using traditional Space Saving, as illustrated in a block diagram in Figure~\ref{fig:LSS_Overview}.
Both components are designed to ensure robustness against prediction errors.






\begin{algorithm}[t]
\caption{\lssplus{} \label{alg:lssplus}}
\begin{algorithmic}[1]
\State \textbf{Initialization}: $T \leftarrow \varnothing$,
\State \textcolor{blue}{$\mathtt{BF}$ -- $\mathtt{Bloom filter}$, $\mathtt{P_{\textit{singleO}}}$ -- $\mathtt{\text{single occurrence predictor}}$}

    \Function{Insert}{$i$}    
    \textcolor{blue}{\If{$\mathtt{P_{singleO}(i) = False}$} \label{lss_plus:line_insertSS}
        \textcolor{black}{\If{$i \in T$}
            \State $c_i \leftarrow c_i + 1$
        \ElsIf{$|T| < k$} \label{line:ss_plus_addentry}
            \State $T \leftarrow T \cup \{i\}$
            \State $c_i \leftarrow 1$
        \Else
            \State $j \leftarrow \text{argmin}_{j \in T} c_j$ 
            \State $c_i \leftarrow c_j + 1$ 
            \State {$T \leftarrow T \cup \{i\} \setminus \{j\}$}
        \EndIf}   
    \Else
        \If{$Uniform(0, 1) \leq \tau$}\Comment{With probability $\tau$}  \label{line:opt1}
        \If{$BF.CONTAINS(i)$}
        \If{$i \in T$}
            \State $c_i \leftarrow c_i + \tau^{-1}$
        \ElsIf{$|T| < k$} \label{line:ssplus_addentry}
            \State $T \leftarrow T \cup \{i\}$
            \State $c_i \leftarrow \tau^{-1}$
        \Else
            \State $j \leftarrow \text{argmin}_{j \in T} c_j$ 
            \State $c_i \leftarrow c_j + \tau^{-1}$ 
            \State {$T \leftarrow T \cup \{i\} \setminus \{j\}$}
        \EndIf
        \Else
        \State $BF.ADD(i)$
        \EndIf
        \EndIf
    \EndIf}
    \EndFunction

    \Function{Query}{$i$}
        \If{$i \in T$}
            \State \Return $c_i$ \textcolor{blue}{$+ \tau^{-1}$} \label{lssplus:line_returncnt}
        \Else
            \State \Return $\min_{j \in T} c_j$ \textcolor{blue}{$+ \tau^{-1}$} \label{lssplus:line_return1}
        \EndIf
    \EndFunction
\end{algorithmic}
\end{algorithm}


\begin{figure*}[t]
	\center{
		\begin{tabular}{ccc}
			\subfloat[IP, Top-k]{\includegraphics[width=\smatrixCellWidth]{graphs/hh/filtersize/aol_topk_precision_vs_filtersize_queryOnW.png}\label{fig:topk_filtersize_web}} &
			\subfloat[IP, HH]{\includegraphics[width=\smatrixCellWidth]{graphs/hh/filtersize/aol_hh_recall_vs_filtersize_queryOnW.png}\label{fig:hh_filtersize_web}}
			\subfloat[Web search, Top-k]{\includegraphics[width=\smatrixCellWidth]{graphs/hh/stream_len/aol_topk_precision_vs_streamlen_queryOnW_full.png}\label{fig:topk_streamlen_web}} 
                \subfloat[Web search, HH]{\includegraphics[width=\smatrixCellWidth]{graphs/hh/stream_len/aol_hh_recall_vs_streamlen_queryOnW_full.png}\label{fig:hh_streamlen_web}}
		\end{tabular}
		}
	\caption{Accuracy vs. filter ratio, precision when finding top-k frequent item when $k=$ and recall when finding heavy hitters with $\theta=$}
	\label{fig:acc_filtersize}
\end{figure*}

